Analyzing the Nuances of Transformers' Polynomial Simplification Abilities

Symbolic Mathematical tasks such as integration often require multiple well-defined steps and understanding of sub-tasks to reach a solution. To understand Transformers' abilities in such tasks in a fine-grained manner, we deviate from traditional end-to-end settings, and explore a step-wise polynomial simplification task. Polynomials can be written in a simple normal form as a sum of monomials which are ordered in a lexicographic order. For a polynomial which is not necessarily in this normal form, a sequence of simplification steps is applied to reach the fully simplified (i.e., in the normal form) polynomial. We propose a synthetic Polynomial dataset generation algorithm that generates polynomials with unique proof steps. Through varying coefficient configurations, input representation, proof granularity, and extensive hyper-parameter tuning, we observe that Transformers consistently struggle with numeric multiplication. We explore two ways to mitigate this: Curriculum Learning and a Symbolic Calculator approach (where the numeric operations are offloaded to a calculator). Both approaches provide significant gains over the vanilla Transformers-based baseline.

==> sections/3_dataset.tex <==

%$\mathcal{P}_0 =  P_1 + P_2 + \ldots +P_{\mathrm{nprod}}$, where $P_i =  \prod_{j=1}^{\mathrm{nfac}_i} f_{ij}$. Here, each factor ($f_{ij}$)  has the form $f = \sum_{k}^{} ({a_k * \prod_{l}^{} x_{kl}^{d_{kl}}})$, where $~x_{kl} \in x_\mathcal{P}$ (dropping $i,j$ for clarity). Here coefficients $ a_{k} \in \mathbb{N}^+$, and powers of the variables $d_{kl} \in \mathbb{N}$. $\mathrm{nprod}$ is the number of products and $\mathrm{nfac}_i$ denotes the number of factors in $P_i$. 
%The simplified endpoint polynomial is of the form $\mathcal{\hat{P}} = \sum_{m=1}^{q} \hat{t}_m$,  where $\hat{t}_m = \hat{a}_m * \prod_{n}^{} {x_n}^{d_{mn}}$, \text{ where } ~$x_n \in x_\mathcal{P}$.
%The symbolic generation using the \texttt{Sympy} library also lets us ensure correctness of each generated expressions and validity of each steps. 

  

% \paragraph{Simplification Steps and Full Proof}
% For both \textsc{coarse} and \textsc{finer} configurations, we build the \textit{proof} steps in the following way: 1) first we do a sequence of \texttt{facstep}s where terms get collected within a factor (such as $2x+3x$ to $5x$, $x^1$ and $1x$ becomes $x$); 2) then a sequence of \texttt{mulstep}s are performed where simplified factors are multiplied out; and 3) lastly, in \texttt{sumstep} simplified products are added together. As mentioned before, the sequence of simplification steps till the endpoint constitute a full \textit{proof}.

%with both \textsc{coarse} and \textsc{finer} simplification steps. For both configurations, three types of simplification are allowed: 1) in \texttt{facstep}, terms get collected within a factor (such as $2x+3x$ to $5x$, $x^1$ and $1x$ becomes $x$); 2) in \texttt{mulstep}, simplified factors are multiplied out, and 3) in \texttt{sumstep} simplified products are added together. For each polynomial, first factor simplification is performed followed by product simplification and then summing of simplified products. As mentioned before, the sequence of simplification steps till the endpoint constitute a full \textit{proof}.\\
%In the \textsc{coarse} configuration, in \texttt{facstep} all the factors in one product are simplified in one step. And similarly, in each \texttt{mulstep} all the simplified factors in one product are multiplied out in one step. In comparison, in the \textsc{finer} configuration, in \texttt{facstep} only one factor gets simplified at each step. Once all factors are simplified, in \texttt{mulstep} only two factors are multiplied at each step. 
% Unsure of this. Human readability is subjective. Maybe we can say "proof-steps that are more aligned with human written proofs". \visheshcomment{The \textsc{coarse} configuration, thus generates more human-readable proofs. Whereas the \textsc{finer} proofs are more detailed but tedious.}
